Microscopic Muscle Image Enhancement

We propose a robust image enhancement algorithm dedicated for muscle fiber specimen images captured by optical microscopes. Blur or out of focus problems are prevalent in muscle images during the image acquisition stage. Traditional image deconvolution methods do not work since they assume the blur kernels are known and also produce ring artifacts. We provide a compact framework which involves a novel spatially non-uniform blind deblurring approach specialized to muscle images which automatically detects and alleviates degraded regions. Ring artifacts problems are addressed and a kernel propagation strategy is proposed to speedup the algorithm and deals with the high non-uniformity of the blur kernels on muscle images. Experiments show that the proposed framework performs well on muscle images taken with modern advanced optical microscopes. Our framework is free of laborious parameter settings and is computationally efficient.

==> alldefin.tex <==
%%%%%%%%  page layout

%\textheight = 8in
%\textwidth = 4.7in
%\evensidemargin= 0.0in
%\oddsidemargin= 0.0in
%\topmargin = - 0.5in
%\headsep = 0.5in
%\columnsep = 0.2in
%\headheight = 0.0in
%\parskip = .1in
%\parindent = 0.4in

%\renewcommand{\labelitemi}{} %{--}

\newcommand{\luv}{$\rm \  L^{*}u^{*}v^{*} \  $}
\newcommand{\lab}{$\rm \  L^{*}a^{*}b^{*} \  $}
\newcommand{\myrfe}[1]{(\ref{eqn:#1})}
\newcommand{\myrff}[1]{\ref{fig:#1}}
\newcommand{\myrfs}[1]{\ref{sec:#1}}
\newcommand{\myrft}[1]{\ref{tab:#1}}
\newcommand{\bo}[1]{{\bf #1}}
\newcommand{\myT}{^{\top}}
\newcommand{\btheta}{\mbox{\boldmath $\theta$}}
\newcommand{\bSigma}{\mbox{\boldmath $\Sigma$}}
\newcommand{\bLambda}{\mbox{\boldmath $\Lambda$}}
\newcommand{\bmu}{\mbox{\boldmath $\mu$}}
\newcommand{\bthetahat}{\mbox{\boldmath $\hat{\theta}$}}
\newcommand{\bthetabar}{\mbox{\boldmath $\bar{\theta}$}}
\newcommand{\myrho}{\rho\left(\left\|\frac{\btheta - \x_{i}}
    {\displaystyle{h}} \right\|^2\right)}
\newcommand{\mypsi}{w \left(\left\|\frac{\bthetahat_j - \x_{i}}
    {\displaystyle{h}} \right\|^2\right)}
\newcommand{\xmypsi}{w \left(\left\|\frac{\bthetahat - \x_{i}}
    {\displaystyle{h}} \right\|^2\right)}

\newcommand{\bu}{\mbox{$\bf u$}}
\newcommand{\bp}{\mbox{$\bf p$}}
\newcommand{\bc}{\mbox{$\bf c$}}
\newcommand{\be}{\mbox{$\bf e$}}

\newcommand{\y}{\mbox{$\bf y$}}
\newcommand{\z}{\mbox{$\bf z$}}
\newcommand{\XS}{\mbox{$\bf\scriptstyle x$}}
\newcommand{\xS}{\mbox{$\bf\scriptstyle x$}}
\newcommand{\zS}{\mbox{$\bf\scriptstyle z$}}
\newcommand{\YS}{\mbox{$\bf\scriptstyle y$}}
\newcommand{\yS}{\mbox{$\bf\scriptstyle y$}}

\newcommand{\f}{\mbox{$\bf f$}}
\newcommand{\0}{\mbox{$\bf 0$}}
\newcommand{\1}{\mbox{$\bf 1$}}
\newcommand{\pp}{\mbox{$\bf p$}}
\newcommand{\qq}{\mbox{$\bf q$}}
\newcommand{\rr}{\mbox{$\bf r$}}
\newcommand{\bs}{\mbox{$\bf s$}}
\newcommand{\s}{\mbox{$\cal{S}_{\x}$}}
\newcommand{\px}{\mbox{$p(\x)$}}
\newcommand{\py}{\mbox{$p(\y)$}}
\newcommand{\R}{\mbox{$\bf R$}}
\newcommand{\T}{\mbox{$\bf T$}}
\newcommand{\B}{\mbox{$\bf B$}}
\newcommand{\C}{\mbox{$\bf C$}}
\newcommand{\E}{\mbox{$\bf E$}}
\newcommand{\G}{\mbox{$\bf G$}}
\newcommand{\J}{\mbox{$\bf J$}}
\newcommand{\LL}{\mbox{$\bf L$}}
\newcommand{\N}{\mbox{$\bf N$}}
\newcommand{\V}{\mbox{$\bf V$}}
\newcommand{\W}{\mbox{$\bf W$}}
\newcommand{\I}{\mbox{$\bf I$}}
\newcommand{\vv}{\mbox{$\bf v$}}
\newcommand{\Myp}{\mbox{\boldmath $\pi$}}
\newcommand{\Mya}{\mbox{\boldmath $\alpha$}}
\newcommand{\Myb}{\mbox{\boldmath $\beta$}}
\newcommand{\MyS}{\mbox{\boldmath $\Sigma$}}
\newcommand{\MyL}{\mbox{\boldmath $\Lambda$}}
\newcommand{\MyP}{\mbox{\boldmath $\Psi$}}
\newcommand{\MyG}{\mbox{\boldmath $\Gamma$}}
\newcommand{\Myo}{\mbox{\boldmath $\omega$}}
\newcommand{\Mu}{\mbox{\boldmath $\mu$}}
\newcommand{\Nu}{\mbox{\boldmath $\nu$}}
\newcommand{\MXi}{\mbox{\boldmath $\xi$}}
\newcommand{\diag}{\mbox{\bf diag}}

\newcommand{\myg}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}}
    \right\|^2\right)}
\newcommand{\mygi}{g\left(\left\|\frac{\x-\x_{i}}{\displaystyle{h}_i}
    \right\|^2\right)}
\newcommand{\mygy}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}}
    \right\|^2\right)}
\newcommand{\mygyi}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h}_i}
    \right\|^2\right)}
\newcommand{\amygy}{g\left(\left\|\frac{\y_j-\x_{i}}{\displaystyle{h_k
    (\y_j )}} \right\|^2\right)}
\newcommand{\mygu}{g\left(\left\|\hat{\y}_u(j+1)-\x_{i}(j+1)\right\|^2\right)}
\newcommand{\myG}{G\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}
\newcommand{\exi}{\mbox{exp}\left(-\left\|\frac{\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxz}{\mbox{exp}\left(-\left\|\frac{\y_j-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\eyxo}{\mbox{exp}\left(-\left\|\frac{\y_{j+1}-\x_i}{\displaystyle{h}}\right\|^2\right)}
\newcommand{\ey}{\mbox{exp}\left(\left\|\frac{\y_{j+1}}{\displaystyle{h}}\right\|^2\right)}

\newcommand{\MSE}{\mbox{MSE}}
\newcommand{\MISE}{\mbox{MISE}}
\newcommand{\var}{\mbox{var}}
\newcommand{\bias}{\mbox{bias}}

\newcommand{\MyI}{\mbox{\boldmath $I$}}
\newcommand{\plim}{\mbox{plim}}


%%%%%%%%  bolds
\newcommand{\hbo}[1]{\hat{{\bf #1}}}

\newcommand{\bhtheta}{\mbox{\boldmath $\hat{\theta}$}}
\newcommand{\halpha}{\hat{\alpha}}
\newcommand{\bbeta}{\mbox{\boldmath $\beta$}}
\newcommand{\bhbeta}{\mbox{\boldmath $\hat{\beta}$}}

\newcommand{\h}{\mbox{$\bf h$}}
\newcommand{\n}{\mbox{$\bf n$}}
\newcommand{\F}{\mbox{$\bf F$}}

\newcommand{\hh}{\hat{h}}

\newcommand{\bx}{{\bf x}}
\newcommand{\by}{{\vc{y}}}  %{{\bf y}}
%\newcommand{\bu}{{\bf u}}
\newcommand{\bv}{{\bf v}}
\newcommand{\bB}{{\bf B}}
\newcommand{\bC}{{\bf C}}
\newcommand{\bH}{{\bf H}}
\newcommand{\M}{{\bf M}}
\newcommand{\bS}{{\bf S}}
\newcommand{\bZ}{{\bf Z}}
\newcommand{\tH}{\widetilde{{\bf H}}}
\newcommand{\HH}{{\bf H}}
\newcommand{\bI}{{\bf I}}
\newcommand{\bW}{{\bf W}}
\newcommand{\Y}{{\bf Y}}
\newcommand{\bY}{{\bf Y}}
\newcommand{\II}{\bo{I}}
\newcommand{\m}{\mbox{$\bf m$}}
\newcommand{\D}{\mbox{$\bf D$}}
\newcommand{\dd}{\mbox{d}}
\newcommand{\X}{\mbox{$\bf X$}}
\newcommand{\Mytheta}{\mbox{\boldmath $\theta$}}
\newcommand{\U}{\mbox{$\bf U$}}
\newcommand{\cc}{\mbox{$\bf c$}}

\newcommand{\Rs}[1]{{\cal R}^{#1}}

%%%%%%%%  operators
\newcommand{\mytr}[1]{{\rm trace} [ #1 ]}
\newcommand{\med}[1]{\mathop{\mbox{med}}\limits_{#1}}
\newcommand{\mymax}[1]{\mathop{\mbox{max}}\limits_{#1}}
\newcommand{\mydet}[1]{{\rm det} [ #1 ]}

\newcommand{\myK}{K\left(\frac{\x-\x_{i}}{\displaystyle{h}}\right)}
\newcommand{\myKy}{K\left(\frac{\y^j-\x_{i}}{\displaystyle{h}}\right)}
\newcommand{\myKD}{K\left(\frac{\x-\x_{D}}{\displaystyle{h}}\right)}
\newcommand{\myKC}{K\left(\frac{\x-\x_{C}}{\displaystyle{h}}\right)}

\newcommand{\myexps}{\mbox{exp}\left(-\frac{1}{2}\|\x\|^2\right)}
\newcommand{\maha}{{\rm D}\left[\x, \x_i, \bH\right]^2}
\newcommand{\mahai}{{\rm D}\left[\x, \x_i, \bH_i\right]^2}
\newcommand{\myexpm}{\mbox{exp}\left(-\frac{1}{2}\maha\right)}
\newcommand{\myexpmi}{\mbox{exp}\left(-\frac{1}{2}\mahai\right)}

\newcommand{\tr}{\mbox{tr\ }}

\newcommand{\myk}{k\left(\left\|\frac{\x_r+\y-\x_{i}}{h}\right\|^2\right)}
\newcommand{\myks}{k\left(\left\|\frac{\x+\y-\x_{i}}{h}\right\|^2\right)}
\newcommand{\mygo}{g\left(\left\|\frac{\x_r+\y_0-\x_{i}}{h}\right\|^2\right)}
\newcommand{\myko}{k\left(\left\|\frac{\x_r+\y_0-\x_{i}}{h}\right\|^2\right)}

\newcommand{\myave}[1]{\mathop{\mbox{ave}}\limits_{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%% below is from matei's part %%%%%%%%%%%%%%%%

%\setlength{\textheight}{9 in}
%\setlength{\textwidth}{6.5in}
\setlength{\baselineskip}{15 pt}

\newcommand{\SSS}{\scriptscriptstyle}
\newcommand{\vc}[1]{\mbox{\boldmath ${#1}$}}

\newcommand{\bbias}{\vc{\mu}}
\newcommand{\htheta}{\mbox{\boldmath $\hat{\theta}$}}
\newcommand{\hhtheta}{\mbox{\boldmath $\Hat{\Hat{\theta}}$}}
\newcommand{\nthetaa}{\mbox{\boldmath $\theta$}}
\newcommand{\ntheta}{\nthetaa_o}
\newcommand{\nalphaa}{\mbox{\boldmath $\alpha$}}
\newcommand{\nalpha}{\nalphaa_o}
%\newcommand{\halpha}{\mbox{\boldmath $\hat{\alpha}$}}
\newcommand{\Nthetaa}{\mbox{\boldmath $\Theta$}}
\newcommand{\Ntheta}{\Nthetaa_o}
\newcommand{\npsii}{\mbox{\boldmath $\psi$}}
\newcommand{\npsi}{\npsii_o}
\newcommand{\hthetaj}{\htheta^{\SSS[j]}}
\newcommand{\hhthetaj}{\hhtheta^{\SSS[j]}}
\newcommand{\hthetaini}{\htheta^{\SSS[0]}}
\newcommand{\hthetajpp}{\htheta^{\SSS[j+1]}}
\newcommand{\hhthetajpp}{\hhtheta^{\SSS[j+1]}}
\newcommand{\hthetajpptop}{\htheta^{{\SSS[j+1]}\,\top}}
\newcommand{\Npsii}{\mbox{\boldmath $\Psi$}}
\newcommand{\Npsi}{\Npsii_o}
\newcommand{\hpsi}{\mbox{\boldmath $\hat{\psi}$}}
\newcommand{\Hpsi}{\mbox{\boldmath $\hat{\Psi}$}}
\newcommand{\Zione}{\vc{Z}_i^{\SSS(1)}}
\newcommand{\Zio}{\vc{Z}_{io}}
\newcommand{\zio}{\vc{z}_{io}}
\newcommand{\hOmegai} {\bhat{\Omega}_i}
\newcommand{\netai}{\vc{\eta}_i}
\newcommand{\Zioneo}{\vc{Z}_{io}^{\SSS(1)}}
\newcommand{\Zioneotop}{\vc{Z}_{io}^{{\SSS(1)}\, \top}}
\newcommand{\Zitwootop}{\vc{Z}_{io}^{{\SSS(2)}\, \top}}
\newcommand{\Zionetop}{\vc{Z}_{i}^{{\SSS(1)}\,\top}}
\newcommand{\Zitwotop}{\vc{Z}_{i}^{{\SSS(2)}\,\top}}
\newcommand{\hZione}{\bhat{Z}_{i}^{\SSS(1)}}
\newcommand{\wione}{\vc{w}_i^{\SSS(1)}}
\newcommand{\wioneo}{\vc{w}_{io}^{\SSS(1)}}
\newcommand{\wi}{\vc{w}_i}
\newcommand{\hwi}{\bhat{w}_i}
\newcommand{\hwione}{\bhat{w}_i^{\SSS(1)}}
\newcommand{\hwitwo}{\bhat{w}_i^{\SSS(2)}}
\newcommand{\tilZione}{\til{Z}_i^{\SSS(1)}}
\newcommand{\tilZone}{\til{Z}^{\SSS(1)}}
\newcommand{\tilZionetop}{\til{Z}_i^{(1)\,\top}}
\newcommand{\wio}{\vc{w}_{io}}
\newcommand{\Zitwo}{\vc{Z}_i^{\SSS(2)}}
\newcommand{\Zitwoo}{\vc{Z}_{io}^{\SSS(2)}}
\newcommand{\witwo}{\vc{w}_i^{\SSS(2)}}
\newcommand{\witwoo}{\vc{w}_{io}^{\SSS(2)}}
\newcommand{\covwi}{\vc{C}_{w_i}}
\newcommand{\covwione}{\vc{C}_{w_i^{\SSS(1)}}}
\newcommand{\nxii}{\mbox{\boldmath $\xi$}}
\newcommand{\nxi}{\nxii_o}
\newcommand{\hxi}{\mbox{\boldmath $\hat{\xi}$}}
\newcommand{\Hxi}{\mbox{\boldmath $\hat{\Xi}$}}
\newcommand{\Htheta}{\mbox{\boldmath $\hat{\Theta}$}}
\newcommand{\Hthetaj}{\Htheta^{\SSS[j]}}
\newcommand{\Hthetajtop}{\Htheta^{{\SSS[j]}\,\top}}
\newcommand{\bvarphi}{\mbox{\boldmath $\varphi$}}
\newcommand{\homega}{\mbox{\boldmath $\hat{\omega}$}}
\newcommand{\nomegaa}{\mbox{\boldmath ${\omega}$}}
\newcommand{\nomega}{\nomegaa_o}
\newcommand{\lik}{\mathcal{L}}
\newcommand{\neps}{\mbox{\boldmath $\epsilon$}}
\newcommand{\hneps}{\mbox{\boldmath $\hat{\epsilon}$}}
\newcommand{\atheta}{\mbox{\boldmath $\bar{\theta}$}}
\newcommand{\trace}{\mbox{tr}}
\newcommand{\ddet}{\mbox{det}}
\newcommand{\vect}{\mbox{\bf vec}}
\newcommand{\dig}{\mbox{\bf diag}}
\newcommand{\bdiag}{\mbox{\bf bdiag}}
%\newcommand{\bias}{\mbox{\bf bias}}
\newcommand{\ith}{i^{\scriptstyle{\mbox{\footnotesize{th}}}}}
\newcommand{\myth}[1]{${#1}^{\scriptstyle{\mbox{\footnotesize{th}}}}$}
\newcommand{\bhat}[1]{\mbox{\boldmath $\hat{#1}$}}
\newcommand{\bbar}[1]{\mbox{\boldmath $\bar{#1}$}}
\newcommand{\btil}[1]{\mbox{\boldmath $\tilde{#1}$}}
\newcommand{\lbhat}[1]{\mbox{\boldmath $\widehat{#1}$}}
\newcommand{\til}[1] {\widetilde{\vc{#1}}}
\newcommand{\vvec}{\mbox{\bf vec}}
\newcommand{\resh}{\mbox{\bf resh}}
\newcommand{\vvecinv}{\resh}
\newcommand{\rank}{\mbox{rank}}
\newcommand{\cov}{\mbox{\bf Cov}}
\newcommand{\rot}{\mbox{\bf rot}}
\newcommand{\PP}{\vc{P}}
\newcommand{\inv}{\,+}
%\newcommand{\rr}{ \mathbb{R}}
\newcommand{\range}{\mathcal{R}}
\newcommand{\nulll}{\mathcal{N}}
\newcommand{\nv}{ \sigma^2_\nu}
\newcommand{\hatnv}{ \hat{\sigma}^2_\nu}
\newcommand{\hatnvml}{ \hat{\sigma}^2_{\nu\SSS(ML)}}
%\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bean}{\begin{eqnarray*}}
\newcommand{\eean}{\end{eqnarray*}}
\newcommand{\ba}{\begin{array}}
\newcommand{\ea}{\begin{array}}
\newcommand{\mydef}{\stackrel{\Delta}{=}}
\newcommand{\Prob}{\mbox{Prob}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Jco}{\Jc(\homega)}
\newcommand{\Jct}{\Jc (\htheta)}
\newcommand{\Jcpsi}{\Jc (\hpsi)}
\newcommand{\Jcat}{\Jc_a(\htheta)}
\newcommand{\Jcao}{\Jc_a(\homega)}
\newcommand{\bUpsilon}{\vc{\Upsilon}}
\newcommand{\bPhi}{\vc{\Phi}}
\newcommand{\bOmega}{\vc{\Omega}}
\newcommand{\nxxi}{\vc{x}_{io}}
\newcommand{\hxxi}{\bhat{x}_{i}}
\newcommand{\xxi}{\vc{x}_i}
\newcommand{\Cxi}{\vc{C}_{x_i}}
\newcommand{\Czi}{\vc{C}_{z_i}}
\newcommand{\Cwi}{\vc{C}_{w_i}}
\newcommand{\Cwihat}{\bhat{C}_{w_i}}
\newcommand{\Cwihatinv}{\bhat{C}_{w_i}^{\inv}}
\newcommand{\Cwiinv}{\vc{C}_{w_i}^{\inv}}
\newcommand{\Cxiinv}{\vc{C}_{x_i}^{\inv}}
\newcommand{\betai}{\vc{\eta}_i}
\newcommand{\jacob}{\vc{J}_{\hat{x}_i}}
\newcommand{\njacob}{\vc{J}_{{x}_{io}}}
\newcommand{\bSigmai}{\bhat{\Sigma}_i}
\newcommand{\bSigmaiinv}{\bhat{\Sigma}_i^{\inv}}
\newcommand{\Zzi}{\vc{Z}_i}
\newcommand{\Zzihat}{\bhat{Z}_i}
\newcommand{\Zzio}{\vc{Z}_{io}}
\newcommand{\bmui}{\bhat{\mu}_{w_i}}
\newcommand{\bzeta}{\vc{\zeta}}
\newcommand{\xlio}{\vc{x}_{io}^l}
\newcommand{\xloneo}{{x}_{1o}^l}
\newcommand{\xltwoo}{{x}_{2o}^l}
\newcommand{\xroneo}{{x}_{1o}^r}
\newcommand{\xrtwoo}{{x}_{2o}^r}

\newcommand{\hxli}{\bhat{x}_{i}^l}
\newcommand{\xli}{\vc{x}_{i}^l}
\newcommand{\cxli}{\btil{x}_{i}^l}

\newcommand{\xliotop}{\vc{x}_{io}^{l\,\top}}
\newcommand{\hxlitop}{\bhat{x}_{i}^{l\,\top}}
\newcommand{\xlitop}{\vc{x}_{i}^{l\,\top}}

\newcommand{\xrio}{\vc{x}_{io}^r}
\newcommand{\hxri}{\bhat{x}_{i}^r}
\newcommand{\xri}{\vc{x}_{i}^r}
\newcommand{\cxri}{\btil{x}_{i}^r}

\newcommand{\xriotop}{\vc{x}_{io}^{r\,\top}}
\newcommand{\hxritop}{\bhat{x}_{i}^{r\,\top}}
\newcommand{\hxriotop}{\bhat{x}_{i}^{r\,\top}}

\newcommand{\Fm}{\vc{F}_o}
\newcommand{\Fhat}{\bhat{F}}
\newcommand{\Fhhat}{\Hat{\Hat{\vc{F}}}}
\newcommand{\meanzi}{\vc{\mu}_{z_i}}
\newcommand{\nzi}{\vc{z}_{io}}
\newcommand{\hzi}{\bhat{z}_{i}}
\newcommand{\bzi}{\vc{z}_{i}}
\newcommand{\alphao}{\alpha_o}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% from leedan's%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\x}{\vc{x}}
\newcommand{\costs}{{J_{s}}}
\newcommand{\costm}{{J_{min}}}
\newcommand{\scost}{J^{\star}}
\newcommand{\ptresh}{P_{\alpha}}
\newcommand{\tresh}{\gamma_{o}}
\newcommand{\hsdd}{\hat{\sigma}_{\nu}^{2}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% newly added

\newcommand{\dirf}{FIG/}
\newcommand{\talpha}{\tilde\alpha}
\newcommand{\tgamma}{\tilde\gamma}
\newcommand{\bgamma}{\mbox{\boldmath $\gamma$}}
\newcommand{\teta}{\tilde\eta}

\newcommand{\myrfss}[1]{\ref{subsec:#1}}
\newcommand{\bpsi}{\mbox{\boldmath $\psi$}}
\newcommand{\myrfc}[1]{\ref{chap:#1}}

\newcommand{\btau}{\mbox{\boldmath $\tau$}}
%\newcommand{\bUpsilon}{\mbox{\boldmath $\Upsilon$}}
\newcommand{\bomega}{\vc{\omega}}

\newcommand{\hby}{\hat{\vc{y}}}
\newcommand{\tby}{\tilde\y}
\newcommand{\tbC}{\tilde{\bf C}}

\newcommand{\tbx}{\tilde{\vc{x}}}
\newcommand{\tbX}{\tilde{\vc{X}}}
\newcommand{\bl}{{\vc{l}}}
\newcommand{\tbe}{\tilde{\vc{e}}}
\newcommand{\bi}{{\vc{i}}}


\newcommand{\bmone}{{$\bf 1$}}

\newcommand{\mykk}{k\left(\left\|\frac{\x-\x_{i}}{h}\right\|^2\right)}

\newcommand{\ww}{{\vc{w}}}
\newcommand{\tbY}{\tilde\Y}

\newcommand{\bb}{\vc{b}}

